DPAUC: Differentially Private AUC Computation in Federated Learning

Federated learning (FL) has gained significant attention recently as a privacy-enhancing tool to jointly train a machine learning model by multiple participants. The prior work on FL has mostly studied how to protect label privacy during model training. However, model evaluation in FL might also lead to potential leakage of private label information. In this work, we propose an evaluation algorithm that can accurately compute the widely used AUC (area under the curve) metric when using the label differential privacy (DP) in FL. Through extensive experiments, we show our algorithms can compute accurate AUCs compared to the ground truth. The code is available at {\url{https://github.com/bytedance/fedlearner/tree/master/example/privacy/DPAUC}}.

==> tables/auc_std_criteo.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[ht!]\centering
% \scriptsize
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{|c|c|c|c|c|c|c}\toprule
AUC and std &$\epsilon$ &$\rho_{+}=\rho_{-}$ &Epoch 1 &Epoch 2 &Epoch 3 \\ \hline
\multirow{10}{*}{\ourapprr{}} &0.1 &47.50\% &0.745667 $\pm$ 2.41$\text{e-}$2 &0.765312 $\pm$ 2.40$\text{e-}$2 &0.777627 $\pm$ 2.62$\text{e-}$2 \\ \cline{2-6}
&0.25 &43.78\% &0.749169 $\pm$ 8.69$\text{e-}$3 &0.767502 $\pm$ 8.76$\text{e-}$3 &0.771198 $\pm$ 7.57$\text{e-}$3 \\ \cline{2-6}
&0.5 &37.75\% &0.749206 $\pm$ 5.39$\text{e-}$3 &0.767081 $\pm$ 4.79$\text{e-}$3 &0.769621 $\pm$ 4.56$\text{e-}$3 \\ \cline{2-6}
&1 &26.89\% &0.749495 $\pm$ 2.11$\text{e-}$3 &0.766833 $\pm$ 2.09$\text{e-}$3 &0.770707 $\pm$ 2.23$\text{e-}$3 \\ \cline{2-6}
&2 &11.92\% &0.749453 $\pm$ 9.43$\text{e-}$4 &0.766621 $\pm$ 8.76$\text{e-}$4 &0.770548 $\pm$ 1.01$\text{e-}$3 \\ \cline{2-6}
&3 &4.74\% &0.749295 $\pm$ 5.46$\text{e-}$4 &0.766490 $\pm$ 4.62$\text{e-}$4 &0.770183 $\pm$ 6.14$\text{e-}$4 \\ \cline{2-6}
&4 &1.80\% &0.749207 $\pm$ 3.75$\text{e-}$4 &0.766458 $\pm$ 3.33$\text{e-}$4 &0.770161 $\pm$ 3.21$\text{e-}$4 \\ \cline{2-6}
&5 &0.67\% &0.749399 $\pm$ 2.05$\text{e-}$4 &0.766477 $\pm$ 2.14$\text{e-}$4 &0.770214 $\pm$ 1.33$\text{e-}$4 \\ \cline{2-6}
&10 &4.54$\text{e-}$5 &0.749383 $\pm$ 1.77$\text{e-}$5 &0.766475 $\pm$ 1.84$\text{e-}$5 &0.770214 $\pm$ 1.67$\text{e-}$5 \\ \cline{2-6}
&$+ \infty$ &0 &0.749383 $\pm$ 0.00$\text{e+}$0 &0.766477 $\pm$ 0.00$\text{e+}$0 &0.770219 $\pm$ 0.00$\text{e+}$0 \\ \hline
scikit-learn &- &0 &0.749383  $\pm$ 1.11$\text{e-}$16  &0.766477 $\pm$ 1.11$\text{e-}$16 &0.770219 $\pm$ 1.11$\text{e-}$16 \\ \hline
Tensorflow &- &0 &0.749382 $\pm$ 5.96$\text{e-}$8 &0.766478 $\pm$ 5.96$\text{e-}$8 &0.770219 $\pm$ 5.96$\text{e-}$8 \\
\hline
\end{tabular}} 
\caption{Mean and standard deviation (std) of AUC computed by \ourapprr{} and ground-truth on the Criteo evaluation set. }
\label{tab:auc_std_criteo}
\end{table*}



==> tables/auc_std_criteo_large.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[ht!]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{|c|c|c|c|c|c|c|}\toprule
&$\epsilon$ &$\rho_{+}=\rho_{-}$ &Epoch 1 &Epoch 2 &Epoch 3 \\ \hline
\multirow{10}{*}{\ourapprr{}} &0.1 &47.50\% &0.751439\ $\pm$ 7.52$\text{e-}$3 &0.768640\ $\pm$ 6.96$\text{e-}$3 &0.774664\ $\pm$ 6.48$\text{e-}$3 \\ \cline{2-6}
&0.25 &43.78\% &0.750405\ $\pm$ 2.90$\text{e-}$3 &0.767958\ $\pm$ 2.85$\text{e-}$3 &0.771694\ $\pm$ 3.26$\text{e-}$3 \\ \cline{2-6}
&0.5 &37.75\% &0.750589\ $\pm$ 1.32$\text{e-}$3 &0.768324\ $\pm$ 1.62$\text{e-}$3 &0.772143\ $\pm$ 1.39$\text{e-}$3 \\ \cline{2-6}
&1 &26.89\% &0.750345\ $\pm$ 5.51$\text{e-}$4 &0.767988\ $\pm$ 7.27$\text{e-}$4 &0.771974\ $\pm$ 8.11$\text{e-}$4 \\ \cline{2-6}
&2 &11.92\% &0.750482\ $\pm$ 3.03$\text{e-}$4 &0.768001\ $\pm$ 3.03$\text{e-}$4 &0.772005\ $\pm$ 3.60$\text{e-}$4 \\ \cline{2-6}
&3 &4.74\% &0.750480\ $\pm$ 1.53$\text{e-}$4 &0.768043\ $\pm$ 1.82$\text{e-}$4 &0.772040\ $\pm$ 1.73$\text{e-}$4 \\ \cline{2-6}
&4 &1.80\% &0.750509\ $\pm$ 9.45$\text{e-}$5 &0.768055\ $\pm$ 1.11$\text{e-}$4 &0.772008\ $\pm$ 1.20$\text{e-}$4 \\ \cline{2-6}
&5 &0.67\% &0.750500\ $\pm$ 5.87$\text{e-}$5 &0.768041\ $\pm$ 6.73$\text{e-}$5 &0.772004\ $\pm$ 6.11$\text{e-}$5 \\ \cline{2-6}
&10 &4.54e-5 &0.750509\ $\pm$ 5.37$\text{e-}$6 &0.768046\ $\pm$ 5.83$\text{e-}$6 &0.772008\ $\pm$ 5.04$\text{e-}$6 \\ \cline{2-6}
&$+\infty$ &0 &0.750509\ $\pm$ 0.00$\text{e+}$0 &0.768045\ $\pm$ 1.11$\text{e-}$16 &0.772007\ $\pm$ 1.11$\text{e-}$16 \\ \hline
scikit-learn &- &0 &0.750509\ $\pm$ 1.11$\text{e-}$16 &0.768045\ $\pm$ 1.11$\text{e-}$16 &0.772007\ $\pm$ 1.11$\text{e-}$16 \\ \hline
Tensorflow &- &0 &0.750509\ $\pm$ 5.96$\text{e-}$8 &0.768044\ $\pm$ 5.96$\text{e-}$8 &0.772006\ $\pm$ 5.96$\text{e-}$8 \\
\bottomrule
\end{tabular}}
\caption{Mean and standard deviation (std) of AUC computed by FedAUC and baselines on large Criteo evaluation set.}\label{tab:auc_std_criteo_large}
\end{table*}

==> tables/auc_std_rr_global_local_adaptive.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c}\toprule
&$\#$ clients &10 &458 &4,584 &45,840 \\ \hline 
&avg. $\#$ data samples per client &45,840.00 &1,000.00 &100.00 &10.00 \\ \hline 
\multirow{6}{*}{$\epsilon=1.0$} &RR &\multicolumn{4}{c}{2.17e-3} \\ \cline{2-6}
&GlobalLaplace &1.22e-4 &8.48e-4 &2.39e-3 &8.08e-3 \\ \cline{2-6}
&LocalLaplace (IID) &1.13e-4 &9.64e-4 &2.26e-3 &7.39e-3 \\ \cline{2-6}
&LocalLaplace (Non-IID) &8.98e-5 &5.29e-4 &1.86e-3 &5.45e-3 \\ \cline{2-6}
&adaptive (IID) &5.15e-5 &3.92e-4 &1.22e-3 &3.80e-3 \\ \cline{2-6}
&LocalLaplace adaptive (Non-IID) &2.93e-5 &1.22e-4 &3.92e-4 &1.03e-3 \\ \hline 
\multirow{6}{*}{$\epsilon=2.0$} &RR &\multicolumn{4}{c}{1.02e-3} \\ \cline{2-6}
&GlobalLaplace &5.85e-5 &4.15e-4 &1.28e-3 &3.95e-3 \\ \cline{2-6}
&LocalLaplace (IID) &5.74e-5 &4.72e-4 &1.21e-3 &4.09e-3 \\ \cline{2-6}
&LocalLaplace (Non-IID) &4.59e-5 &2.91e-4 &9.45e-4 &3.09e-3 \\ \cline{2-6}
&LocalLaplace adaptive (IID) &2.60e-5 &1.84e-4 &6.48e-4 &1.66e-3 \\ \cline{2-6}
&LocalLaplace adaptive (Non-IID) &1.59e-5 &6.01e-5 &1.52e-4 &5.54e-4 \\ \hline 
\multirow{6}{*}{$\epsilon=4.0$} &RR &\multicolumn{4}{c}{3.49e-4} \\ \cline{2-6}
&GlobalLaplace &2.92e-5 &2.09e-4 &6.58e-4 &1.88e-3 \\ \cline{2-6}
&LocalLaplace (IID) &3.11e-5 &1.94e-4 &5.80e-4 &1.86e-3 \\ \cline{2-6}
&LocalLaplace (Non-IID) &2.49e-5 &1.48e-4 &4.44e-4 &1.53e-3 \\ \cline{2-6}
&LocalLaplace adaptive (IID) &1.36e-5 &8.20e-5 &2.87e-4 &9.08e-4 \\ \cline{2-6}
&LocalLaplace adaptive (Non-IID) &7.80e-6 &2.81e-5 &8.72e-5 &2.77e-4 \\ \hline 
\multirow{6}{*}{$\epsilon=8.0$} &RR &\multicolumn{4}{c}{4.41e-5} \\ \cline{2-6}
&GlobalLaplace &1.54e-5 &9.82e-5 &3.31e-4 &1.05e-3 \\ \cline{2-6}
&LocalLaplace (IID) &1.51e-5 &1.06e-4 &3.27e-4 &8.52e-4 \\ \cline{2-6}
&LocalLaplace (Non-IID) &1.06e-5 &6.99e-5 &2.19e-4 &7.50e-4 \\ \cline{2-6}
&LocalLaplace adaptive (IID) &7.01e-6 &4.55e-5 &1.37e-4 &4.61e-4 \\ \cline{2-6}
&LocalLaplace adaptive (Non-IID) &3.89e-6 &1.36e-5 &4.34e-5 &1.38e-4 \\
\bottomrule
\end{tabular}}
\caption{Standard deviation of AUC estimated by different methods (DP budget allocation $\alpha = 0.5$ which means that $\epsilon_{\text{localSum}} = \epsilon_{\text{localP}} = 0.5\epsilon$). IID: assigned samples to clients uniformly. Non-IID: assigned samples to clients based on their prediction scores.}\label{tab:std_auc_rr_global_local_adaptive}
\end{table}

==> tables/auc_std_w_accurate_number_of_positive_and_negative_samples.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[ht!]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & avg. $\#$ data samples per client &45,840 &458.4 &4.6 &1 \\ \hline
\multirow{3}{*}{$\epsilon=1.0$} &GlobalLaplace &- &4.84e-5 &5.26e-4 &4.45e-3 &1.10e-2 \\ \cline{2-7}
&\multirow{2}{*}{LocalLaplace} &i.i.d &4.81e-5 &4.66e-4 &4.25e-3 &6.44e-3 \\
& &\cellcolor[HTML]{A8A8A8}non i.i.d &\cellcolor[HTML]{A8A8A8}3.40e-5 &\cellcolor[HTML]{A8A8A8}2.98e-4 &\cellcolor[HTML]{A8A8A8}2.76e-3 &\cellcolor[HTML]{A8A8A8}6.08e-3 \\  \hline
\multirow{3}{*}{$\epsilon=2.0$} &GlobalLaplace &- &2.61e-5 &2.58e-4 &2.37e-3 &5.65e-3 \\ \cline{2-7}
&\multirow{2}{*}{LocalLaplace} &i.i.d &2.61e-5 &2.48e-4 &2.10e-3 &2.87e-3 \\
& &\cellcolor[HTML]{A8A8A8}non i.i.d &\cellcolor[HTML]{A8A8A8}1.48e-5 &\cellcolor[HTML]{A8A8A8}1.51e-4 &\cellcolor[HTML]{A8A8A8}1.38e-3 &\cellcolor[HTML]{A8A8A8}3.20e-3 \\  \hline
\multirow{3}{*}{$\epsilon=4.0$} &GlobalLaplace &- &1.30e-5 &1.21e-4 &1.21e-3 &2.68e-3 \\ \cline{2-7}
&\multirow{2}{*}{LocalLaplace} &i.i.d &1.23e-5 &1.20e-4 &1.14e-3 &1.56e-3 \\
& &\cellcolor[HTML]{A8A8A8}non i.i.d &\cellcolor[HTML]{A8A8A8}6.63e-6 &\cellcolor[HTML]{A8A8A8}7.22e-5 &\cellcolor[HTML]{A8A8A8}6.20e-4 &\cellcolor[HTML]{A8A8A8}1.69e-3 \\  \hline
\multirow{3}{*}{$\epsilon=8.0$} &GlobalLaplace &- &6.29e-6 &5.94e-5 &6.12e-4 &1.34e-3 \\ \cline{2-7}
&\multirow{2}{*}{LocalLaplace} &i.i.d &5.79e-6 &6.32e-5 &5.07e-4 &8.09e-4 \\
& &\cellcolor[HTML]{A8A8A8}non i.i.d &\cellcolor[HTML]{A8A8A8}3.98e-6 &\cellcolor[HTML]{A8A8A8}3.70e-5 &\cellcolor[HTML]{A8A8A8}3.44e-4 &\cellcolor[HTML]{A8A8A8}8.53e-4 \\
\bottomrule
\end{tabular}}
\caption{Standard deviation of estimated AUC with accurate $P$ and $N$. i.i.d: assigned samples to clients uniformly. non i.i.d: assigned samples to clients based on their prediction scores.}\label{tab:std_auc_w_accurate_P_and_N}
\end{table*}

==> tables/auc_std_w_noisy_number_of_positive_and_negative_samples.tex <==

\begin{table}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
&$\#$ clients &10 &458 &1,000 &4,584 &45,840 &100,000 &458,407 \\ \hline 
&avg. $\#$ data samples per client &45,840.00 &1,000.00 &458.40 &100.00 &10.00 &4.60 &1 \\ \hline 
\multirow{4}{*}{$\epsilon=1.0$} &RR &\multicolumn{7}{c}{2.17e-3} \\ \cline{2-9}
&GlobalLaplace &1.22e-4 &8.48e-4 &1.24e-3 &2.39e-3 &8.08e-3 &1.24e-2 &2.77e-2 \\ \cline{2-9}
&LocalLaplace (IID) &1.13e-4 &9.64e-4 &1.26e-3 &2.26e-3 &7.39e-3 &1.10e-2 &1.99e-2 \\ \cline{2-9}
&\cellcolor[HTML]{A8A8A8}LocalLaplace (Non-IID) &\cellcolor[HTML]{A8A8A8}8.98e-5 &\cellcolor[HTML]{A8A8A8}5.29e-4 &\cellcolor[HTML]{A8A8A8}8.49e-4 &\cellcolor[HTML]{A8A8A8}1.86e-3 &\cellcolor[HTML]{A8A8A8}5.45e-3 &\cellcolor[HTML]{A8A8A8}8.33e-3 &\cellcolor[HTML]{A8A8A8}1.81e-2 \\ 
&adaptive (IID) &5.15e-5 &3.92e-4 & & 1.22e-3& 3.80e-3& & \\ \cline{2-9}
&adaptive (non-IID) &2.93e-5 &1.22e-4 & & 3.92e-4& 1.03e-3& & \\ \cline{2-9}
\hline 
\multirow{4}{*}{$\epsilon=2.0$} &RR &\multicolumn{7}{c}{1.02e-3} \\ \cline{2-9} 
&GlobalLaplace &5.85e-5 &4.15e-4 &5.62e-4 &1.28e-3 &3.95e-3 &5.21e-3 &1.32e-2 \\ \cline{2-9} 
&LocalLaplace (IID) &5.74e-5 &4.72e-4 &5.78e-4 &1.21e-3 &4.09e-3 &5.24e-3 &8.86e-3 \\ \cline{2-9}
&\cellcolor[HTML]{A8A8A8}LocalLaplace (Non-IID) &\cellcolor[HTML]{A8A8A8}4.59e-5 &\cellcolor[HTML]{A8A8A8}2.91e-4 &\cellcolor[HTML]{A8A8A8}4.93e-4 &\cellcolor[HTML]{A8A8A8}9.45e-4 &\cellcolor[HTML]{A8A8A8}3.09e-3 &\cellcolor[HTML]{A8A8A8}4.38e-3 &\cellcolor[HTML]{A8A8A8}9.96e-3 \\ 
&adaptive (IID) & 2.60e-5&1.84e-4 & & 6.48e-4& 1.66e-3& & \\ \cline{2-9}
&adaptive (non-IID) & 1.59e-5&6.01e-5 & & 1.52e-4& 5.54e-4& & \\ \cline{2-9}
\hline 
\multirow{4}{*}{$\epsilon=4.0$} &RR &\multicolumn{7}{c}{3.49e-4} \\ \cline{2-9} 
&GlobalLaplace &2.92e-5 &2.09e-4 &3.26e-4 &6.58e-4 &1.88e-3 &3.22e-3 &7.02e-3 \\ \cline{2-9} 
&LocalLaplace (IID) &3.11e-5 &1.94e-4 &3.00e-4 &5.80e-4 &1.86e-3 &2.40e-3 &4.38e-3 \\ \cline{2-9}
&\cellcolor[HTML]{A8A8A8}LocalLaplace (Non-IID) &\cellcolor[HTML]{A8A8A8}2.49e-5 &\cellcolor[HTML]{A8A8A8}1.48e-4 &\cellcolor[HTML]{A8A8A8}2.05e-4 &\cellcolor[HTML]{A8A8A8}4.44e-4 &\cellcolor[HTML]{A8A8A8}1.53e-3 &\cellcolor[HTML]{A8A8A8}2.26e-3 &\cellcolor[HTML]{A8A8A8}4.39e-3 \\ 
&adaptive (IID) & 1.36e-5&8.20e-5 & & 2.87e-4& 9.08e-4& & \\ \cline{2-9}
&adaptive (non-IID) & 7.80e-6&2.81e-5 & & 8.72e-5& 2.77e-4& & \\ \cline{2-9}
\hline 
\multirow{4}{*}{$\epsilon=8.0$} &RR &\multicolumn{7}{c}{4.41e-5} \\ \cline{2-9}
&GlobalLaplace &1.54e-5 &9.82e-5 &1.53e-4 &3.31e-4 &1.05e-3 &1.58e-3 &2.99e-3 \\\cline{2-9}
&LocalLaplace (IID) &1.51e-5 &1.06e-4 &1.40e-4 &3.27e-4 &8.52e-4 &1.35e-3 &2.29e-3 \\\cline{2-9}
&\cellcolor[HTML]{A8A8A8}LocalLaplace (Non-IID) &\cellcolor[HTML]{A8A8A8}1.06e-5 &\cellcolor[HTML]{A8A8A8}6.99e-5 &\cellcolor[HTML]{A8A8A8}1.14e-4 &\cellcolor[HTML]{A8A8A8}2.19e-4 &\cellcolor[HTML]{A8A8A8}7.50e-4 &\cellcolor[HTML]{A8A8A8}1.16e-3 &\cellcolor[HTML]{A8A8A8}2.22e-3 \\
&adaptive (IID) &7.01e-6 &4.55e-5 & & 1.37e-4& 4.61e-4& & \\ \cline{2-9}
&adaptive (non-IID) &3.89e-6 &1.36e-5 & & 4.34e-5& 1.38e-4& & \\ \cline{2-9}
\hline 
\bottomrule
\end{tabular}}
\caption{Standard deviation of AUC estimated by different methods (DP budget allocation $\alpha = 0.5$ which means that $\epsilon_{\text{localSum}} = \epsilon_{\text{localP}} = 0.5\epsilon$). IID: assigned samples to clients uniformly. Non-IID: assigned samples to clients based on their prediction scores.}\label{tab:std_auc_w_noisy_P_and_N}
\end{table}


==> tables/dpauc/dp_auc_non_iid_clients_1000_thresholds_100.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
epoch &Tensorflow &scikit-learn &$\epsilon'$=0.02, $\epsilon$=8 &$\epsilon'$=0.01, $\epsilon$=4 &$\epsilon'$=0.005, $\epsilon$=2 &$\epsilon'$=0.0025,$\epsilon$=1 \\ \hline 
0 &0.749357 &0.749383 &0.748062 $\pm$ 0.001981 &0.746105 $\pm$ 0.004465 &0.741711 $\pm$ 0.009246 &0.726885 $\pm$ 0.016539 \\
1 &0.766434 &0.766477 &0.764923 $\pm$ 0.002036 &0.763246 $\pm$ 0.004022 &0.756715 $\pm$ 0.009105 &0.744978 $\pm$ 0.018234 \\
2 &0.770189 &0.770219 &0.768894 $\pm$ 0.002104 &0.766819 $\pm$ 0.003802 &0.759916 $\pm$ 0.007251 &0.746815 $\pm$ 0.016511 \\
\bottomrule
\end{tabular}}
\caption{Non-IID setting with $K=1,000$ and $|\Theta|=100$. }\label{tab:dpauc_non_iid_clients_1000_thresholds_100}
\end{table*}

==> tables/dpauc/dpauc_iid_clients_1000_thresholds_100.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
epoch &Tensorflow &scikit-learn &$\epsilon'$=0.02, $\epsilon$=8 &$\epsilon'$=0.01, $\epsilon$=4 &$\epsilon'$=0.005, $\epsilon$=2 &$\epsilon'$=0.0025,$\epsilon$=1 \\ \hline 
0 &0.749357 &0.749383 &0.74811 $\pm$ 0.002335 &0.745557 $\pm$ 0.004498 &0.738944 $\pm$ 0.008008 &0.726187 $\pm$ 0.014704 \\
1 &0.766434 &0.766477 &0.764887 $\pm$ 0.002241 &0.763012 $\pm$ 0.004378 &0.756938 $\pm$ 0.008096 &0.740619 $\pm$ 0.017457 \\
2 &0.770189 &0.770219 &0.76918 $\pm$ 0.002519 &0.766482 $\pm$ 0.004387 &0.761074 $\pm$ 0.007947 &0.745812 $\pm$ 0.014596 \\
\bottomrule
\end{tabular}}
\caption{IID setting with $K=1,000$ and $|\Theta|=100$}\label{tab:dpauc_iid_clients_1000_thresholds_100}
\end{table*}

==> tables/dpauc/dpauc_iid_clients_10_thresholds_10.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
epoch &Tensorflow &scikit-learn &$\epsilon'=0.2$, $\epsilon=8$ &$\epsilon'=0.1$, $\epsilon=4$ &$\epsilon'=0.05$, $\epsilon=2$ &$\epsilon'=0.025$, $\epsilon=1$ \\ \hline 
0 &0.749357 &0.749383 &0.7251052 $\pm$ 0.000074 &0.725064 $\pm$ 0.000167 &0.725008 $\pm$ 0.000323 &0.724899 $\pm$ 0.000607 \\
1 &0.766434 &0.766477 &0.744348 $\pm$ 0.000084 &0.744317 $\pm$ 0.000144 &0.744215 $\pm$ 0.000328 &0.744058 $\pm$ 0.000639 \\
2 &0.770189 &0.770219 &0.748858 $\pm$ 0.000073 &0.7487984 $\pm$ 0.000123 &0.748821 $\pm$ 0.000331 &0.748626 $\pm$ 0.000591 \\
\bottomrule
\end{tabular}}
\caption{IID setting with $K=10$ and $|\Theta|=10$}\label{tab:dpauc_iid_clients_10_thresholds_10}
\end{table*}

==> tables/dpauc/dpauc_iid_clients_10_thresholds_100.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
epoch &Tensorflow &scikit-learn &$\epsilon'$=0.02, $\epsilon$=8 &$\epsilon'$=0.01, $\epsilon$=4 &$\epsilon'$=0.005, $\epsilon$=2 &$\epsilon'$=0.0025,$\epsilon$=1 \\ \hline 
0 &0.749357 &0.749383 &0.749347 $\pm$ 0.000216 &0.749178 $\pm$ 0.000484 &0.748937 $\pm$ 0.000755 &0.748206 $\pm$ 0.001649 \\
1 &0.766434 &0.766477 &0.766373 $\pm$ 0.000239 &0.766309 $\pm$ 0.000402 &0.76611 $\pm$ 0.000894 &0.765684 $\pm$ 0.001677 \\
2 &0.770189 &0.770219 &0.770091 $\pm$ 0.000258 &0.769995 $\pm$ 0.000498 &0.770028 $\pm$ 0.000788 &0.769143 $\pm$ 0.00172 \\
\bottomrule
\end{tabular}}
\caption{IID setting with $K=10$ and $|\Theta|=100$}\label{tab:dpauc_iid_clients_10_thresholds_100}

\end{table*}

==> tables/dpauc/dpauc_iid_clients_10_thresholds_200.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
epoch &Tensorflow &scikit-learn &$\epsilon$=0.01, $\epsilon$=8 &$\epsilon$=0.005, $\epsilon$=4 &$\epsilon$=0.0025,$\epsilon$=2 &$\epsilon$=0.00125,$\epsilon$=1 \\
0 &0.749357 &0.749383 &0.74929 $\pm$ 0.000289 &0.74916 $\pm$ 0.000573 &0.748491 $\pm$ 0.001204 &0.747117 $\pm$ 0.002224 \\
1 &0.766434 &0.766477 &0.76638 $\pm$ 0.000311 &0.766235 $\pm$ 0.000677 &0.765694 $\pm$ 0.001367 &0.764399 $\pm$ 0.002264 \\
2 &0.770189 &0.770219 &0.770137 $\pm$ 0.000319 &0.769729 $\pm$ 0.000633 &0.769066 $\pm$ 0.001085 &0.767694 $\pm$ 0.002746 \\
\bottomrule
\end{tabular}}
\caption{IID setting with $K=10$ and $|\Theta|=200$}\label{tab:dpauc_iid_clients_10_threholds_200}
\end{table*}

==> tables/dpauc/dpauc_iid_clients_10_thresholds_25.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
epoch &Tensorflow &scikit-learn &$\epsilon'=0.08$, $\epsilon=8$ &$\epsilon'=0.04$, $\epsilon=4$ &$\epsilon'=0.02$, $\epsilon=2$ &$\epsilon'=0.01$, $\epsilon=1$ \\ \hline 
0 &0.749357 &0.749383 &0.747879 $\pm$ 0.000147 &0.747895 $\pm$ 0.000275 &0.747669 $\pm$ 0.000625 &0.747278 $\pm$ 0.000889 \\
1 &0.766434 &0.766477 &0.765178 $\pm$ 0.000159 &0.765045 $\pm$ 0.000252 &0.7649144 $\pm$ 0.000507 &0.764968 $\pm$ 0.001282 \\
2 &0.770189 &0.770219 &0.769006 $\pm$ 0.000162 &0.768992 $\pm$ 0.000323 &0.768705 $\pm$ 0.000508 &0.768357 $\pm$ 0.001308 \\
\bottomrule
\end{tabular}}
\caption{IID Setting with $K=10$ and $|\Theta| = 25$}\label{tab:dpauc_iid_clients_10_thresholds_25}
\end{table*}

==> tables/dpauc/dpauc_iid_clients_10_thresholds_50.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering

\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
epoch &Tensorflow &scikit-learn &$\epsilon$=0.04, $\epsilon$=8 &$\epsilon$=0.02, $\epsilon$=4 &$\epsilon$=0.01, $\epsilon$=2 &$\epsilon$=0.005, $\epsilon$=1 \\ \hline 
0 &0.749357 &0.749383 &0.748914 $\pm$ 0.000161 &0.748884 $\pm$ 0.000343 &0.748988 $\pm$ 0.000657 &0.748816 $\pm$ 0.001279 \\
1 &0.766434 &0.766477 &0.766198 $\pm$ 0.000187 &0.766181 $\pm$ 0.000329 &0.765973 $\pm$ 0.000723 &0.766009 $\pm$ 0.001216 \\
2 &0.770189 &0.770219 &0.769806 $\pm$ 0.000220 &0.769756 $\pm$ 0.000500 &0.769549 $\pm$ 0.000805 &0.76939 $\pm$ 0.001034 \\
\bottomrule
\end{tabular}}
\caption{IID setting with $K=10$ and $|\Theta|=50$}\label{tab:dpauc_iid_clients_10_thresholds_50}
\end{table*}

==> tables/dpauc/dpauc_non_iid_clients_10_thresholds_100.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize 
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c|c}\toprule
& & &\multicolumn{4}{c}{DPAUC} \\ \hline 
\textbf{epoch} &Tensorflow &scikit-learn &$\epsilon'$=0.02, $\epsilon$=8 &$\epsilon'$=0.01, $\epsilon$=4 &$\epsilon'$=0.005, $\epsilon$=2 &$\epsilon'$=0.0025,$\epsilon$=1 \\ \hline
\textbf{0} &0.749357 &0.749383 &0.749319 $\pm$ 0.000242 &0.749260 $\pm$ 0.000474 &0.749192 $\pm$ 0.00072 &0.748962 $\pm$ 0.00178 \\
\textbf{1} &0.766434 &0.766477 &0.766378 $\pm$ 0.000231 &0.766197 $\pm$ 0.000471 &0.76612 $\pm$ 0.000755 &0.765447 $\pm$ 0.001805 \\
\textbf{2} &0.770189 &0.770219 &0.770095 $\pm$ 0.000213 &0.770115 $\pm$ 0.000434 &0.76981 $\pm$ 0.000903 &0.769265 $\pm$ 0.001502 \\
\bottomrule
\end{tabular}}
\caption{Non-IID setting with $K= 10$ and $|\Theta = 100|$}\label{tab:dpauc_non_iid_clients_10_thresholds_100}
\end{table*}

==> tables/evaluation_set_statistics.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[ht!]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{|c|c|c|c|c|}\toprule
& $\#$ Positives ($P$) & $\#$ Negatives ($N$) & $\#$ Total ($M$) \\ \hline
Small Criteo Evaluation Set &117,317 &341,090 &458,407 \\ \hline
Large Criteo Evaluation Set &1,173,981 &3,410,081 &4,584,062 \\ 
\bottomrule
\end{tabular}}
\caption{Statistics of Two Criteo Evaluation Sets}\label{tab:evaluation_set_statistics}
\end{table*}

==> tables/evaluation_set_statistics_partial.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{|c|c|c|c|c|}\toprule
& $\#$ Positives ($P$) & $\#$ Negatives ($N$) & $\#$ Total ($M$) \\ \hline
 Criteo Evaluation Set &117,317 &341,090 &458,407 \\ 
\bottomrule
\end{tabular}}
\caption{Statistics of Criteo Evaluation Set}\label{tab:evaluation_set_statistics_criteo_partial}
\end{table*}

==> tables/noisy_auc_only_randomized_response.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[ht!]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c|c|c}\toprule
AUC &$\epsilon$ &$\rho_{+}=\rho_{-}$ &Epoch 1 &Epoch 3 &Epoch 3 \\ \hline 
\multirow{6}{*}{Noisy AUC} &0.1 &47.50\% &0.509429 &0.510137 &0.510237 \\  \cline{2-6}
&0.5 &37.75\% &0.546986 &0.550344 &0.550862 \\ \cline{2-6}
&1 &26.89\% &0.592421 &0.598951 &0.600010 \\ \cline{2-6}
&2 &11.92\% &0.667666 &0.679436 &0.681911 \\ \cline{2-6}
&4 &1.80\% &0.735230 &0.751306 &0.754892 \\ \cline{2-6}
&10 &4.54e-5 &0.749343 &0.766438 &0.770177 \\ \hline 
scikit-learn &- &0 &0.749383 &0.766477 &0.770219 \\ \hline 
Tensorflow &- &0 &0.749382 &0.766478 &0.770219 \\
\bottomrule
\end{tabular}}
\caption{Noisy AUC computed by Randomized Response mechanism without debiasing.}\label{tab:noisy_auc_randomized_response_wo_converting}
\scriptsize
\end{table}

==> tables/top_k_analysis_production_data.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c}\toprule
Top K & $\#$ Positives in Top K &Precision &Recall \\ \hline
1 &0 &0 &0 \\ \hline
5 &2 &0.4 &1.20e-3 \\ \hline
10 &2 &0.2 &1.20e-3 \\ \hline
50 &6 &0.12 &3.70e-3 \\ \hline
100 &13 &0.13 &8.00e-3 \\ \hline
500 &50 &0.1 &0.0306 \\ \hline
1,000 &94 &0.094 &0.0576 \\ \hline
5,000 &326 &0.0652 &0.1998 \\ \hline
10,000 &525 &0.0525 &0.3217 \\ \hline
50,000 &1,339 &0.0268 &0.8205 \\ \hline
100,000 &1,632 &0.0163 &1 \\
\bottomrule
\end{tabular}}
\caption{Top-k analysis on private data}\label{tab:top_k_analysis_production_data}
% \scriptsize
\end{table*}

==> tex/method_ll.tex <==
\section{Proposed Algorithm 2: Laplace and Gaussian Mechanism}
\label{sec:method_2}

% \kevin{Why is it local?}
In this section, we introduce how to compute the AUC with label differential privacy by leveraging Laplace and Gaussian mechanism. Here we use Laplace mechanism as an example. Other settings for the Gaussian mechanism will be the same. 

\subsection{Overall Workflow}
The workflow of this method is as shown in Figure ~\ref{fig:fedauc_illustration_lap} in the appendix and the detailed  Algorithm is shown in Algorithm ~\ref{alg:clients_server_cal_auc_2} in the Appendix. The algorithm has four steps (the first two steps are the same as \ourapprr{}):
 
\begin{enumerate}[leftmargin=*]
    \item \textbf{Clients Execute.} Each client $C_k$ computes the prediction scores $s_k = f(X_k)$ for all its owning data points and sends shuffled $s^k$ to the server.  
    \item \textbf{Server Executes.} The server aggregates all the prediction scores and sort them in an increasing order. Each prediction score $s_i^k$ ($i \in [1, M]$) will be assigned a ranking order $r_i^k$. %The instance with the highest order will be assigned $r = M - 1$, and the second highest one will be assigned $M -2$ and so on. The smallest ranking score is $r = 0$. 
    The server sends each ranking order $r_i^k$ back to the corresponding client $C_k$ which owns $s_i^k$. 
    \item \textbf{Clients Execute.} Each client $C_k$ then aggregates all its received ranking orders with its label. The corresponding result is $\text{localSum}_k = \sum_{i}^{|{Y_k}|} r_i^k \cdot {y_i}$, where $y_i$ is the ground-truth label. The client also computes its number of  positive ($\text{localP}$) and negative ($\text{localN}$) instances respectively. Here $\text{localP} = \sum_{i}^{|{Y_k}|} {y_i}$ and  $\text{localN} = \sum_{i}^{|{Y_k}|} (1- {y_i}) $. Each client $C_k$ adds noise to $\text{localSum}_k$ and $\text{localP}_k$ to get  $\text{localSum}_k'$ and $\text{localP}_k'$ respectively. The client $C_k$ sends $\text{localSum}_k'$, $\text{localP}_k'$, and  $\text{localN}_k'$ ($\text{localN}_k' = |Y_k| - \text{localP}_k'$) to the  server. We talk about how to add noises to these local statistics in Section ~\ref{sec:adding_noise_to_local_statistics}.
    \item \textbf{Server Executes.} After receiving all clients' $\text{localSum}'$, $\text{localP}'$ and $\text{localN}'$, the server aggregates them to get the corresponding global values. Here $\text{globalSum} = \sum_{k}^K \text{localSum}_k'$, $\bar{P} = \sum_{k}^K \text{localP}_k'$, and $\bar{N} = \sum_{k}^K \text{localN}_k'$. The server then leverages equation ~\eqref{eq:auc_ranking} to compute the AUC. The final AUC is: $\text{AUC} = \frac{{\text{globalSum} - {\bar{P}(\bar{P}-1)}/{2}}}{{\bar{P}\bar{N}}}$.
\end{enumerate}


\subsection{Adding Noise to Local Statistics}
\label{sec:adding_noise_to_local_statistics}

We explain in details how to perturb $\text{localSum}$ and $\text{localP}$ for each client in the algorithm. Both Gaussian and Laplace mechanisms can be leveraged to generate the corresponding DP noise. Without loss of generality, we use Laplace as an example. Laplace mechanism preserves $(\epsilon, 0)$-differential privacy if the random noise is drawn from $Lap(\Delta/\epsilon)$ where $\Delta$ is the $l_1$ sensitivity. We name this method as \ourapplap{}. The noise is added as the following:

\begin{enumerate}[leftmargin=*]
    \item Adding noise to $\text{localSum}$: Each client $C_k$ decides its own sensitivity by selecting its maximum ranking order as $\Delta_{\text{localSum}^k} = \max_{i \in [1, |Y_k|]}(r_i^k)$. Given a privacy budget $\epsilon_{localSum}$, client $C_k$ draws the random noise from $\textsf{Lap}(\Delta_{\text{localSum}^k}/\epsilon_{localSum})$.
    \item Adding noise to $\text{localP}$: Each client $C_k$ sets $\Delta_{\text{localP}^k} = 1$. Given a privacy budget $\epsilon_{localP}$, client $C_k$ draws the random noise from $\textsf{Lap}(1/\epsilon_{localP})$.
\end{enumerate}

\para{Privacy Analysis.}
The total privacy budget $\epsilon =\epsilon_{localSum} + \epsilon_{localP}$. We use a parameter $\alpha$ to control the budget allocation: $\epsilon_{localSum} = \alpha \epsilon$ and $\epsilon_{localP} = (1- \alpha) \epsilon$. Next we explain  a better allocation than using $\alpha$.

\subsection{Adaptive Allocation of DP Budget} 
\label{sec:adaptive_allocation_of_dp_budget} 

Finding $\alpha$ that achieves a good tradeoff between utility and privacy can be difficult and would require many trials and errors if using cross validation. Therefore we propose an algorithm that automatically determines the allocation of the DP budget adaptively on each client.

% Is there a way to do the allocation of the DP budget adaptive on each client? 


\input{tex/orthogonal_decomposition}









==> tex/method_rr.tex <==


\section{Proposed Algorithm 1: Randomized Response Mechanism}
\label{sec:methods}

% In this section, we introduce how to compute the AUC with label differential privacy in federated learning by leveraging randomized response. We name this method as \ourapprr{}. The workflow of this method is as shown .

We introduce our first algorithm to compute AUC when applying label DP to vFL for evaluation. The algorithm is based on randomized response~\cite{RR} and we name it as \ourapprr{}. We include the workflow in Figure ~\ref{fig:fedauc_illustration_rr} in the Appendix. We now explain the algorithm step by step.

% \begin{figure*}[h!]
% % \vspace{-0.1in}
% \captionsetup[subfigure]{labelformat=empty}
%   \begin{subfigure}{0.49\linewidth}
%   \centering
%     \includegraphics[width=1.0\linewidth]{figures/FederatedAUCComputation.pdf}
%       \caption{(a): Illustration of our proposed \ourapp{} with randomized response. }
%   \end{subfigure}
%   \begin{subfigure}{0.49\linewidth}
%   \centering
%     \includegraphics[width=1.0\linewidth]{figures/FederatedAUCComputation_2.pdf}
%     \caption{(b): Illustration of our proposed \ourapp{} with Gaussian or Laplace mechanism.}
%   \end{subfigure}
%   \caption{.}
%  \label{fig:workflow_of_fedauc} 
%  \end{figure*}
 

\subsection{Step 1: Clients Flip Their Local Labels}


Randomized response (RR) is $\epsilon$-LabelDP and  works as following: let $\epsilon$ be a parameter and let $y \in \{0, 1\}$ be the true label. Given a query of $y$, RR will respond with a random draw $\tilde{y}$ from the following probability distribution: 
%value known to the $\text{RR}_\epsilon$. \xin{what is $\text{RR}_\epsilon$?}When an observer queries the value of $y$, $\text{RR}_\epsilon$ responds with a random draw $\tilde{y}$ from the following probability distribution:

% Randomized response (RR) is $\epsilon$-LabelDP and  defined as following: let $\epsilon$ be a parameter and let $y \in \{0, 1\}$ be the true label value known to the $\text{RR}_\epsilon$. \xin{what is $\text{RR}_\epsilon$?}When an observer queries the value of $y$, $\text{RR}_\epsilon$ responds with a random draw $\tilde{y}$ from the following probability distribution:

\begin{equation}
\label{eq:rr}
    \Pr[\tilde y = \hat y] = \begin{cases}
     \frac{e^\epsilon}{1+e^\epsilon} & \text{for $y = \hat y$,} \\
    \frac{1}{1+e^\epsilon} & \text{otherwise.}
                            \end{cases}
\end{equation}


% \begin{definition}[RR is $\epsilon$-LabelDP]
% The above version of RR is $(\epsilon, 0)$-LabelDP, since we have:

% \begin{align*}
%     \frac{\Pr[\tilde y = 1|y=1]}{\Pr[\tilde y = 1|y=0]} = \frac{\frac{e^\epsilon}{1+e^\epsilon}}{\frac{1}{1+e^\epsilon}} = e^\epsilon = \frac{\Pr[\tilde y = 0|y=0]}{\Pr[\tilde y = 0|y=1]} 
% \end{align*}

% And we have $\delta = 0$. Hence RR is $\epsilon$-LabelDP as desired. 
% \end{definition}

Clients can leverage randomized response (Algorithm ~\ref{alg:clients_flipping_labels} in the Appendix) to flip their owning labels as a preprocessing step before computing the AUC. It's worth mentioning that all labels are only flipped once and the generated noisy labels can then be used for further evaluations multi-times. 

% \xin{\eqref{eq:rr} itself is the randomized response mechanism. No need for reference to appendix. Also this is not pre-processing. It is one step of the algorithm. Finally, the wording is too close to \cite{labeldp21}}

\subsection{Step 2: Server Computes AUC from Flipped Labels}
\label{sec:corr_auc}

We now talk about how to compute the AUC with the flipped labels (detailed description can be seen in Algorithm ~\ref{alg:clients_server_cal_auc} in the Appendix). 
 Since the corresponding AUC is computed with flipped labels,
 we denote this AUC as \emph{noisy AUC}: $\text{AUC}^{D_\text{noisy}}$. It has four steps:

\begin{enumerate}[leftmargin=*]
    \item \textbf{Clients Execute.} Suppose we have $K$ clients. Each client $C_k$ computes the prediction scores $s_k = f(X_k)$ for all its owning data points and sends shuffled $s^k$ to the server.  
    \item \textbf{Server Executes.} The server aggregates all the prediction scores and sort them in an increasing order. Each prediction score $s_i^k$ ($i \in [1, M]$) will be assigned a ranking order $r_i^k$. The instance with the highest order will be assigned $r = M - 1$, and the second highest one will be assigned $M -2$ and so on. The smallest ranking score is $r = 0$. The server sends each ranking order $r_i^k$ back to the corresponding client $C_k$ which owns $s_i^k$. %It's worth mentioning the prediction scores have to be shared with the server for some tasks. For example, the clients have to report the predicted conversion rate (CVR) of the ad impression to the server in online advertisements. The server can later on calculate the bid price by multiplying the predicted CVR with  a constant parameter tuned according to the campaign budget and performance ~\cite{bidding2018}. Then the server can select the advertiser who proposed the highest bid price as the winner to show the ad. 
    \item \textbf{Clients Execute.} Each client $C_k$ then aggregates all its received ranking orders with the noisy label generated in Algorithm ~\ref{alg:clients_flipping_labels}. The corresponding result is $\text{localSum}_k = \sum_{i}^{|{Y_k}|} r_i^k \cdot {y_i}'$, where $y_i'$ is the flipped version of ground-truth label $y_i$. The client also computes its number of noisy positive ($\text{localP}$) and negative ($\text{localN}$) instances respectively. Here $\text{localP} = \sum_{i}^{|{Y_k}|} {y_i}'$ and  $\text{localN} = \sum_{i}^{|{Y_k}|} (1- {y_i}') $.
    Each client $C_k$ sends its $\text{localSum}_k$, $\text{localP}_k$, and $\text{localN}_k$ to the server. 
    \item \textbf{Server Executes.} After receiving all clients' $\text{localSum}$, $\text{localP}$ and $\text{localN}$, the server aggregates them to get the corresponding global values. Here $\text{globalSum} = \sum_{k}^K \text{localSum}_k$, $\bar{P} = \sum_{k}^K \text{localP}_k$, and $\bar{N} = \sum_{k}^K \text{localN}_k$. The server then leverages equation ~\eqref{eq:auc_ranking} to compute the AUC. We then get the corresponding noisy AUC: $\text{AUC}^{D_{\text{noisy}}} = \frac{{\text{globalSum} - {\bar{P}(\bar{P}-1)}/{2}}}{{\bar{P}\bar{N}}}$.
\end{enumerate}

% The detailed description of the corresponding algorithm can be seen in Algorithm ~\ref{alg:clients_server_cal_auc}. 
It's possible that the clients can send their flipped labels and corresponding prediction scores to the server directly and the server then computes $\text{AUC}^{D_{\text{noisy}}}$ in a centralized way. Both methods will get the same value of the noisy AUC. To be consistent with our other mechanisms, we instead introduce the one with four steps here.


\subsection{Step 3: Server Debiases AUC}
\label{sec:covert_auc_to_real}

Section ~\ref{sec:corr_auc} shows how the server compute $\text{AUC}^{D_{\text{noisy}}}$ with using clients' local flipped labels. Empirically, the noisy AUC can be useless with a small privacy budget $\epsilon$ (see experimental results in Table ~\ref{tab:noisy_auc_randomized_response_wo_converting} in the Appendix). In this section, we show how to covert  $\text{AUC}^{D_{\text{noisy}}}$ to the final AUC that we are interested in and we name it as $\text{AUC}^{D_{\text{clean}}}$. 
$\text{AUC}^{D_{\text{clean}}}$ is a more accurate estimation of the ground-truth AUC than $\text{AUC}^{D_{\text{noisy}}}$.


\cite{ConvertAUC2015} proposed to learn from noisy binary labels via class-probability estimation. They draw $(X, Y) \sim D$. The instance $X$ is unchanged: however, the label is altered such that positive samples have labels flipped with probability $\rho_{+}$, while negative samples have labels flipped with probability $\rho_{-}$. %The AUC computed based on the noisy labels is noted as $\text{AUC}^{D_{\text{noisy}}}$, 
We note the AUC computed based on the ground-truth labels as $\text{AUC}^{D_{\text{clean}}}$. \cite{ConvertAUC2015} proved the following relation between $\text{AUC}^{D_{\text{noisy}}}$ and $\text{AUC}^{D_{\text{clean}}}$:

\begin{equation}
\label{equ:auc_convertion}
  \text{AUC}^{D_{\text{clean}}}  =  \frac{\text{AUC}^{D_{\text{noisy}}} - \frac{\alpha+\beta}{2}}{1-\alpha-\beta}    
\end{equation}

where 
\begin{equation}
    \label{equ:alpha_beta}
    \alpha = \frac{(1-\pi) \rho_{-}}{\pi(1-\rho_{+}) + (1-\pi)\rho_{-}}, \quad 
    \beta = \frac{\pi \rho_{+}}{\pi \rho_{+} + (1-\pi)(1-\rho_{-})}
\end{equation}

Here $\pi = P_{D}(Y=1)$ is the positive ratio (base rate) in the clean data $D$. $\pi$ is unknown to the server. However, the server can estimate $\pi$ from the known information of the noisy data $D'$. Suppose we observe $\bar{M}$ positive examples and $\bar{N}$ negative examples in the noisy data $D'$. We then estimate $\pi$ as $\pi' = \frac{P'}{P' + N'}$ where $P'$ and $N'$ are estimated positive and negative numbers in the clean data $D$. And they can be estimated as $P' = \frac{\bar{P}(1-\rho_{-}) - \bar{N}\rho_{-}}{1-\rho_{+}-\rho_{-}}$, and $\quad N'= \bar{P}+\bar{N}-P'$. More details can be in Section ~\ref{sec:estimate_pi} of the Appendix.


% \begin{equation}
%     P'+N' = \bar{P}+\bar{N}, \quad P'(1-\rho_{+}) + N \rho_{-} = \bar{P}
% \end{equation}





After we get get $\text{AUC}^{D_{\text{noisy}}}$ and $\pi'$, we can leverage equation ~\eqref{equ:alpha_beta} to compute $\alpha$ and $\beta$, and then use equation ~\ref{equ:auc_convertion} to get the $\text{AUC}^{D_{\text{clean}}}$ that we are interested in. Algorithm ~\ref{alg:real_auc_from_corr} in the Appendix shows how the server compute $\text{AUC}^{D_{\text{clean}}}$ from  $\text{AUC}^{D_{\text{noisy}}}$, $\bar{P}$, $\bar{N}$, and Label DP budget $\epsilon$.



\para{Privacy and Utility Analysis.}
Our proposed approach is $\epsilon$-LabelDP since all of operations are on the noisy labels flipped by randomized response which is $\epsilon$-LabelDP. We include the utility (variance of computed AUC) analysis in Section~\ref{sec:utility_rr} of the Appendix.

% \subsection{Utility analysis}

% We now have:

% \begin{equation}
% \label{eq:std_of_noisy_auc_w_accurate_p_n}
% \begin{split}
% \textbf{Var}(AUC^{D_{\text{noisy}}})  \\ = \textbf{Var}(\frac{\sum^K sum_i - \frac{P * (P-1)}{2}}{P * N})  =  \textbf{Var}(\frac{\sum^K sum_i}{P * N}) \\= \textbf{Var}(\frac{\sum_{i=1}^P s_i (1-r)+\sum_{j=1}^N s_j r}{P * N}) \\= \frac{\sum_{i=1}^{M}s_i^2 r  (1-r)}{P^2 * N^2} = \frac{r(1-r)\sum_{i=1}^{M-1}i^2}{P^2 * N^2} \\
% = r(1-r)\frac{M(M-1)(2M-1)/6}{P^2 * N^2} \\
% = \frac{exp(\epsilon)}{(1+exp(\epsilon))^2}\frac{M(M-1)(2M-1)/6}{P^2 * N^2}
% \end{split}
% \end{equation}



==> tex/orthogonal_decomposition.tex <==
Our inspiration comes from the special case where each client only owns 1 sample, i.e., $|Y_k|=1$ for each client $C_k$.
In this case, 
it turns out that $\text{localSum}_k = r^k \cdot \text{localP}_k$. Since $r^k$ is public, we do not need to generate two independent random variables;
we can sample $s\sim \mathsf{Lap}(1/\epsilon)$,
and report $\text{localP}_k':=\text{localP}_k+s$ and $\text{localSum}_k':=r^k\cdot \text{localP}_k'$.

The above example shows that when $\text{localSum}_k$ and $\text{localP}_k$ are highly correlated, then the privacy budget can be allocated more efficiently.
Based on this observation, we can analyze the general case.
Fix the client $C_k$.
Let $\mathbf{y}:=(y_1,\cdots,y_{|Y_k|})\in \{0,1\}^{|Y_k|}$ be the labels held by $C_k$,
and $\mathbf{r}:=(r_1^k,\cdots,r_{|Y_k|}^k)\in \mathbb{Z}^{|Y_k|}$ be their rankings.
Then we have $\text{localP}_k=\langle \mathbf{u},\mathbf{y}\rangle$ and $\text{localSum}_k = \langle \mathbf{r},\mathbf{y}\rangle$,
where $\mathbf{u}:=(1,1,\cdots,1)$ is the all-one vector.

When $\mathbf{u}$ and $\mathbf{r}$ are parallel, namely $\mathbf{r} = r\cdot \mathbf{u}$ for some $r\in \mathbb{R}$,
we can still allocate all the budget on $\text{localP}_k'$,
and report $\text{localSum}_k'=r\cdot \text{localP}_k'$.
Otherwise,
we can decompose $\mathbf{r}$ into two orthogonal components:
we can write $\mathbf{r}:=\mathbf{u}'+\mathbf{v}'$ where $\mathbf{u}'\parallel \mathbf{u}$ and $\mathbf{u}'\perp \mathbf{v'}$.
Then we have 
\begin{align*}
    \text{localSum}_k=\langle \mathbf{r},\mathbf{y}\rangle = \langle \mathbf{u'},\mathbf{y}\rangle+\langle \mathbf{v'},\mathbf{y}\rangle.
\end{align*}
In order to make $(\text{localP}_k,\text{localSum}_k)$ $\epsilon$-DP,
by the post-processing property of differential privacy,
it is sufficient to have $(\langle \mathbf{u}',y\rangle, \langle \mathbf{v}',y\rangle)$ to be $\epsilon$-DP. We can use a parameter $\beta$ to control the budget allocation so that $\langle \mathbf{u}',y\rangle$ achieves $\beta \epsilon$-DP and $\langle \mathbf{v}',y\rangle$ achieves $(1-\beta)\epsilon$-DP.
If we use Laplace mechanism, this means we sample $s_1\sim \mathsf{Lap}(1/(\beta \epsilon))$ and $s_2\sim \mathsf{Lap}(1/((1-\beta)\epsilon))$,
and report $\text{localP}_k':=\langle \mathbf{u},y\rangle+s_1$,
$\text{localSum}_k':=\langle \mathbf{u}',y\rangle+\|\mathbf{u}'\|_{\infty}\cdot s_1+\langle \mathbf{v}',y\rangle+\|\mathbf{v}'\|_{\infty}\cdot s_2$.

We can tune the parameter $\beta$ to achieve small standard deviation of estimated AUC. However, the server may need additional validation data to select a optimal $\beta$ which performs the best. Sometimes, it is impractical in the setting of FL. We now show how to adaptively choose the allocation parameter $\beta$ for each client.
Simply, we use the heuristic of choosing $\beta$ that minimizes the variance of $\text{localSum}_k'$ for client $k$,
which is equivalent to minimizing the variance of $\|\mathbf{u}'\|_{\infty}\cdot s_1+\|\mathbf{v}'\|_{\infty}\cdot s_2$.
